RWKV-edge: Deeply Compressed RWKV for Resource-Constrained Devices

To deploy LLMs on resource-contained platforms such as mobile robots and smartphones, non-transformers LLMs have achieved major breakthroughs. Recently, a novel RNN-based LLM family, Repentance Weighted Key Value (RWKV) has shown strong computational efficiency; nevertheless, RWKV models still have high parameter counts which limited their deployment. In this paper, we propose a suite of compression techniques, ranging from model architecture optimizations to post-training compression, tailored to the RWKV architecture. Combined, our techniques reduce the memory footprint of RWKV models by 3.4x -- 5x with only negligible degradation in accuracy; compared to transformer LLMs with similar accuracy, our models require 4x less memory footprint.

==> fig-ablation-mem.tex <==
% !TeX root = main.tex
\begin{figure}
    \begin{subfigure}[t]{0.40\textwidth}
	\centering
	\includegraphics[width=1\textwidth]{figs/ablation-mem}
	\caption{}
	\label{fig:ablation-mem}
    \end{subfigure}
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[page=1,width=1\textwidth]{figs/results-sparsity-predictor}
        \caption{}
        \label{fig:results-sparsity-predictor}
    \end{subfigure}
    \caption{(a) Memory reduction rate of each technique on different model sizes.
    (SVD = Singular Value Decomposition, CLS = the clustered head, Sparse = sparsity for the channel-mix layer) (b) Accuracy and sparsity rate achieved by the ground-truth (GT) and quantized predictors ($n$-bit). }
\end{figure}


==> fig-mem-i8.tex <==
% !TeX root = main.tex
\begin{figure}
	\centering
	\includegraphics[width=0.48\textwidth]{figs/scripts/fig_i8_acc_memlayer.pdf}
	\caption{TBD}
	\label{fig:mem-usage}
\end{figure}


==> fig-memlayer.tex <==
% !TeX root = main.tex
\begin{figure}
	\centering
	\includegraphics[width=0.48\textwidth]{figs/scripts/fig_acc_memlayer_official.pdf}
	\caption{
        lambada\_openai's accuracy and models' in-memory usage in layerwise.
        Our models (w/ red edge line) have the smallest memory footprint as layerwise.
	}
	\label{fig:memlayer_official}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.48\textwidth]{figs/scripts/fig_acc_memlayer_pretrain.pdf}
	\caption{
        lambada\_openai's accuracy and models' in-memory usage in layerwise.
        Our models (w/ red edge line) have the smallest memory footprint as layerwise.
	}
	\label{fig:memlayer_pretrain}
\end{figure}


==> fig-other-models.tex <==
% !TeX root = main.tex
\begin{table}
	\centering
	\caption{Comparison of accuracy between baselines.}
	\includegraphics[width=0.48\textwidth]{figs/dummy}
	\label{fig:other-models}
\end{table}


==> fig-param-dist.tex <==
% !TeX root = main.tex
\begin{figure}
	\centering
	\includegraphics[width=0.47\textwidth]{figs/param-dist}
	\caption{Parameter distribution of the official models.}
	\label{fig:param-dist}
\end{figure}


==> fig-template.tex <==
% !TeX root = main.tex
\begin{figure}
	\centering
	\includegraphics[width=0.48\textwidth]{figs/dummy}
	\caption{}
	\label{fig:dummy}
\end{figure}


==> tab-tfacc.tex <==
% !TeX root = main.tex
\begin{table}
	\centering
	\caption{Accuracy and perplexity results of the transformer and RWKV models. A displayed task is lambada\_openai.}
	\includegraphics[width=0.48\textwidth]{figs/tfacc}
	\label{tab:tfacc}
\end{table}

